A Tale of Trust and Accuracy: Base vs. Instruct LLMs in RAG Systems

Retrieval Augmented Generation (RAG) represents a significant advancement in artificial intelligence combining a retrieval phase with a generative phase, with the latter typically being powered by large language models (LLMs). The current common practices in RAG involve using "instructed" LLMs, which are fine-tuned with supervised training to enhance their ability to follow instructions and are aligned with human preferences using state-of-the-art techniques. Contrary to popular belief, our study demonstrates that base models outperform their instructed counterparts in RAG tasks by 20% on average under our experimental settings. This finding challenges the prevailing assumptions about the superiority of instructed LLMs in RAG applications. Further investigations reveal a more nuanced situation, questioning fundamental aspects of RAG and suggesting the need for broader discussions on the topic; or, as Fromm would have it, "Seldom is a glance at the statistics enough to understand the meaning of the figures".

==> figures/prompt_base.tex <==
\begin{figure}[ht]
 % Options: \small, \tiny, \scriptsize, \footnotesize, \small, \normalsize
% \begin{figure}[h!]
\begin{tcolorbox}[title=Base LLM - Llama 2 7B]
\emph{You are given a question and you MUST respond by EXTRACTING the answer from one of the provided documents. If none of the documents contain the answer, respond with NO-RES.}\\

\textbf{Documents:}\\
\textbf{Document [1]}(Title: Batman Returns) the Penguin. We didn't really officially cast it, but for a short nasty little guy, it's a short list. I ended up writing the character for Danny DeVito." \textcolor{correct}{Burgess Meredith} (who portrayed the Penguin in the 1960s TV series "Batman") was cast for a little cameo as Tucker Cobblepot...\\
\textbf{Document [2]}(Title: Batman: Mystery of the Batwoman) This is the only time in the DC animated universe that Paul Williams did not voice the Penguin...\\
\textbf{Document [3]}(Title: The Penguin's a Jinx) The Penguin goes to Wayne Manor and returns the actress. He then uses his gas-umbrella to knock out anyone inside the statues...
\\ \\
\textbf{Question:} Who played the part of `The Penguin' in the TV series `Batman'?

\textbf{Answer:} \textcolor{correct}{Burgess Meredith}
\end{tcolorbox} 
\caption{}

\label{fig:prompt_related_gold}
\end{figure}





==> figures/prompt_instruct.tex <==
\begin{figure*}[htbp]
% \begin{figure}[h!]
\begin{tcolorbox}[title=Instruct LLM - Llama 2 7B-Chat]
\emph{You are given a question and you MUST respond by EXTRACTING the answer from one of the provided documents. If none of the documents contain the answer, respond with NO-RES.}\\

\textbf{Documents:}\\
\textbf{Document [1]}(Title: Batman Returns) the Penguin. We didn't really officially cast it, but for a short nasty little guy, it's a short list. I ended up writing the character for Danny DeVito." \textcolor{correct}{Burgess Meredith} (who portrayed the Penguin in the 1960s TV series "Batman") was cast for a little cameo as Tucker Cobblepot...\\
\textbf{Document [2]}(Title: Batman: Mystery of the Batwoman) This is the only time in the DC animated universe that Paul Williams did not voice the Penguin. This film marked the final performance of John Vernon as Rupert Thorne before his death in 2005...\\
\textbf{Document [3]}(Title: The Penguin's a Jinx) The Penguin goes to Wayne Manor and returns the actress. He then uses his gas-umbrella to knock out anyone inside the statues...
\\ \\
\textbf{Question:} Who played the part of `The Penguin' in the TV series `Batman'?

\textbf{Answer:} Document [3](Title: The Penguin's a Jinx) - \textcolor{red}{The Penguin's a Jinx}
\end{tcolorbox} 
\caption{}

\label{fig:prompt_related_gold}
\end{figure*}

==> figures/prompt_template.tex <==
\begin{figure*}[htbp]
% \begin{figure}[h!]
\begin{tcolorbox}[title=Instruct + Template LLM - Llama 2 7B-Chat + Template]
\emph{[INST] <<SYS>> \\
You are given a question and you MUST respond by EXTRACTING the answer from one of the provided documents. If none of the documents contain the answer, respond with NO-RES.\\
<</SYS>>}\\

\textbf{Documents:}\\
\textbf{Document [1]}(Title: Batman Returns) the Penguin. We didn't really officially cast it, but for a short nasty little guy, it's a short list. I ended up writing the character for Danny DeVito." \textcolor{correct}{Burgess Meredith} (who portrayed the Penguin in the 1960s TV series "Batman") was cast for a little cameo as Tucker Cobblepot...\\
\textbf{Document [2]}(Title: Batman: Mystery of the Batwoman) This is the only time in the DC animated universe that Paul Williams did not voice the Penguin...\\
\textbf{Document [3]}(Title: The Penguin's a Jinx) The Penguin goes to Wayne Manor and returns the actress. He then uses his gas-umbrella to knock out anyone inside the statues...
\\ \\
\textbf{Question:} Who played the part of `The Penguin' in the TV series `Batman'?

\textbf{Answer:} \emph{[/INST]} Based on the provided documents, the answer to the question "Who played the part of `The Penguin' in the TV series `Batman'?" is \textcolor{red}{Danny DeVito}
\end{tcolorbox} 
\caption{}

\label{fig:prompt_related_gold}
\end{figure*}

==> tables/nq_first_prompt.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table*}[ht]
% \centering
% \caption{NQ plain}
% \label{tab:nq_first}
% \begin{tabular}{@{}l|cccccccc@{}}
% \toprule
% \multicolumn{1}{c|}{\textbf{NQ}}    & \multicolumn{8}{c}{\textbf{\# Retrieved Documents}}                                      \\ \midrule
% \multicolumn{1}{c|}{\textbf{Model}} & Closed-Book              & 1              & 2              & 3     & 4     & 5     & 8     & 10    \\ \midrule
% Llama 2 7B          & \textbf{25.20} & \textbf{23.88} & \textbf{24.71} & \textbf{27.83} & \textbf{29.53} & \textbf{30.22} & \textbf{31.01} & \textbf{31.46} \\
% Llama 2 7B-Chat                     & 16.51          & 16.06          & 18.48          & 18.62 & 18.59 & 19.21 & 21.98 & 21.08 \\
% Llama 2 7B-Chat + Template          & 13.12          & 3.36           & 1.21           & 0.69  & 0.48  & 0.45  & 0.73  & 1.52  \\ \midrule
% Llama 3 8B          & 22.01          & \textbf{27.03} & \textbf{30.22} & \textbf{30.53} & \textbf{31.08} & \textbf{29.08} & \textbf{29.49} & \textbf{28.70} \\
% Llama 3 8B-Instruct                 & 27.17          & 8.52           & 10.25          & 15.40 & 15.85 & 22.57 & 28.80 & 28.25 \\
% Llama 3 8B-Instruct + Template      & \textbf{27.80} & 14.40          & 17.34          & 19.04 & 15.30 & 18.10 & 20.35 & 19.35 \\ \midrule
% Mistral 7B                          & \textbf{28.11} & \textbf{24.26} & \textbf{25.30} & 25.72 & 26.17 & 27.66 & 26.65 & 28.87 \\
% Mistral 7B-Instruct & 18.76          & 20.04          & 24.99          & \textbf{26.69} & \textbf{30.56} & \textbf{31.67} & \textbf{33.33} & \textbf{34.82} \\
% Mistral 7B-Instruct + Template      & 15.96          & 18.17          & 23.54          & 19.14 & 27.90 & 27.45 & 27.07 & 26.79 \\ \midrule
% Falcon 7B           & \textbf{15.26} & \textbf{17.13} & \textbf{18.97} & \textbf{21.15} & \textbf{21.08} & \textbf{21.95} & \textbf{22.64} & \textbf{22.33} \\
% Falcon 7B-Instruct                  & 12.74          & 15.68          & 17.72          & 17.96 & 19.21 & 20.08 & 20.04 & 20.98 \\ \bottomrule
% \end{tabular}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[ht]
\centering
\caption{NQ plain}
\label{tab:nq_first}
\begin{tabular}{@{}l|ccccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{NQ}}    & \multicolumn{7}{c}{\textbf{\# Retrieved Documents}}                                                                  \\ \midrule
\multicolumn{1}{c|}{\textbf{Model}} & 1              & 2              & 3              & 4              & 5              & 8              & 10             \\ \midrule
Llama 2 7B                          & \textbf{23.88} & \textbf{24.71} & \textbf{27.83} & \textbf{29.53} & \textbf{30.22} & \textbf{31.01} & \textbf{31.46} \\
Llama 2 7B-Chat                     & 16.06          & 18.48          & 18.62          & 18.59          & 19.21          & 21.98          & 21.08          \\
Llama 2 7B-Chat + Template          & 3.36           & 1.21           & 0.69           & 0.48           & 0.45           & 0.73           & 1.52           \\ \midrule
Llama 3 8B                          & \textbf{27.03} & \textbf{30.22} & \textbf{30.53} & \textbf{31.08} & \textbf{29.08} & \textbf{29.49} & \textbf{28.70} \\
Llama 3 8B-Instruct                 & 8.52           & 10.25          & 15.40          & 15.85          & 22.57          & 28.80          & 28.25          \\
Llama 3 8B-Instruct + Template      & 14.40          & 17.34          & 19.04          & 15.30          & 18.10          & 20.35          & 19.35          \\ \midrule
Mistral 7B                          & \textbf{24.26} & \textbf{25.30} & 25.72          & 26.17          & 27.66          & 26.65          & 28.87          \\
Mistral 7B-Instruct                 & 20.04          & 24.99          & \textbf{26.69} & \textbf{30.56} & \textbf{31.67} & \textbf{33.33} & \textbf{34.82} \\
Mistral 7B-Instruct + Template      & 18.17          & 23.54          & 19.14          & 27.90          & 27.45          & 27.07          & 26.79          \\ \midrule
Falcon 7B                           & \textbf{17.13} & \textbf{18.97} & \textbf{21.15} & \textbf{21.08} & \textbf{21.95} & \textbf{22.64} & \textbf{22.33} \\
Falcon 7B-Instruct                  & 15.68          & 17.72          & 17.96          & 19.21          & 20.08          & 20.04          & 20.98          \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/nq_second_prompt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[ht]
\centering
\caption{NQ with proof}
\label{tab:nq_second}
\begin{tabular}{@{}l|ccccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{NQ}}    & \multicolumn{7}{c}{\textbf{\# Retrieved Documents}}                                                                  \\ \midrule
\multicolumn{1}{c|}{\textbf{Model}} & 1              & 2              & 3              & 4              & 5              & 8              & 10             \\ \midrule
Llama 2 7B                          & \textbf{24.82} & \textbf{28.70} & \textbf{31.71} & \textbf{32.85} & \textbf{34.09} & \textbf{35.62} & \textbf{35.79} \\
Llama 2 7B-Chat                     & 18.41          & 24.96          & 28.76          & 30.22          & 32.16          & 33.16          & 32.05          \\
Llama 2 7B-Chat + Template          & 1.59           & 2.42           & 3.88           & 5.75           & 8.45           & 12.81          & 12.91          \\ \midrule
Llama 3 8B                          & \textbf{29.39} & \textbf{31.53} & \textbf{34.72} & \textbf{37.07} & \textbf{36.59} & \textbf{39.15} & \textbf{40.22} \\
Llama 3 8B-Instruct                 & 18.83          & 23.57          & 25.65          & 27.97          & 30.84          & 34.13          & 37.97          \\
Llama 3 8B-Instruct + Template      & 11.70          & 16.44          & 6.40           & 6.61           & 11.60          & 5.64           & 0.69           \\ \midrule
Mistral 7B                          & \textbf{24.82} & \textbf{30.74} & \textbf{33.75} & \textbf{35.17} & \textbf{36.83} & \textbf{40.15} & \textbf{40.15} \\
Mistral 7B-Instruct                 & 21.53          & 27.66          & 29.91          & 32.85          & 33.58          & 36.45          & 35.76          \\
Mistral 7B-Instruct + Template      & 16.86          & 18.10          & 20.87          & 22.43          & 24.09          & 24.44          & 26.96          \\ \midrule
Falcon 7B                           & \textbf{17.58} & \textbf{20.04} & \textbf{22.43} & \textbf{23.75} & \textbf{23.85} & \textbf{26.12} & \textbf{26.72} \\
Falcon 7B-Instruct                  & 16.10          & 18.31          & 18.93          & 19.87          & 20.91          & 21.61          & 21.30          \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/nq_second_prompt_coherence.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[ht]
\centering
\label{tab:nq_second_coherence}
\caption{NQ coherence percentage with proof}
\begin{tabular}{@{}l|ccccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{NQ}}    & \multicolumn{7}{c}{\textbf{\# Retrieved Documents}}                              \\ \midrule
\multicolumn{1}{c|}{\textbf{Model}} & 1     & 2     & 3     & 4              & 5     & 8              & 10             \\ \midrule
Llama 2 7B                          & 36.93 & 41.16 & 41.64 & 41.43          & 42.16 & \textbf{42.99} & \textbf{41.26} \\
Llama 2 7B-Chat     & \textbf{45.07} & \textbf{47.35} & \textbf{46.97} & \textbf{46.45} & \textbf{45.17} & 40.53          & 32.78          \\
Llama 2 7B-Chat + Template          & 0     & 0.59  & 1.14  & 0.07           & 0.07  & 0              & 0              \\ \midrule
Llama 3 8B                          & 36.90 & 41.36 & 43.54 & \textbf{46.49} & 46.80 & \textbf{51.78} & 51.37          \\
Llama 3 8B-Instruct & \textbf{42.02} & \textbf{51.92} & \textbf{50.71} & 43.86          & \textbf{48.36} & 48.29          & \textbf{53.10} \\
Llama 3 8B-Instruct + Template      & 0.52  & 0.03  & 0.10  & 0.14           & 1.38  & 0.28           & 0.07           \\ \midrule
Mistral 7B                          & 36.73 & 44.03 & 46.56 & 45.66          & 51.47 & 54.62          & 53.31          \\
Mistral 7B-Instruct & \textbf{50.12} & \textbf{53.24} & \textbf{54.38} & \textbf{55.49} & \textbf{57.39} & \textbf{57.74} & \textbf{56.07} \\
Mistral 7B-Instruct + Template      & 15.99 & 10.90 & 7.65  & 5.75           & 3.53  & 4.12           & 2.70           \\ \midrule
Falcon 7B                           & 1.87  & 2.08  & 3.32  & 3.01           & 3.81  & 4.50           & 1.15           \\
Falcon 7B-Instruct  & \textbf{3.39}  & \textbf{3.12}  & \textbf{3.77}  & \textbf{4.85}  & \textbf{4.26}  & \textbf{1.73}  & \textbf{1.04}  \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/triviaqa_first_prompt.tex <==

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table*}[ht]
% \centering
% \caption{TriviaQA plain}
% \label{tab:trivia_first}
% \begin{tabular}{@{}l|crrrrrrr@{}}
% \toprule
% \multicolumn{1}{c|}{\textbf{TriviaQA}} &
%   \multicolumn{8}{c}{\textbf{\# Retrieved Documents}} \\ \midrule
% \multicolumn{1}{c|}{\textbf{Model}} &
%   Closed-Book &
%   \multicolumn{1}{c}{1} &
%   \multicolumn{1}{c}{2} &
%   \multicolumn{1}{c}{3} &
%   \multicolumn{1}{c}{4} &
%   \multicolumn{1}{c}{5} &
%   \multicolumn{1}{c}{8} &
%   \multicolumn{1}{c}{10} \\ \midrule
% Llama 2 7B &
%   \textbf{55.57} &
%   \textbf{55.85} &
%   \textbf{57.15} &
%   \textbf{59.28} &
%   \textbf{60.40} &
%   \textbf{61.24} &
%   \textbf{62.93} &
%   \textbf{63.89} \\
% Llama 2 7B-Chat &
%   37.33 &
%   32.59 &
%   34.63 &
%   41.09 &
%   42.95 &
%   46.14 &
%   49.19 &
%   48.96 \\
% Llama 2 7B-Chat + Template &
%   41.73 &
%   23.35 &
%   21.63 &
%   21.13 &
%   17.70 &
%   18.05 &
%   22.30 &
%   25.68 \\ \midrule
% Llama 3 8B &
%   \textbf{57.37} &
%   \textbf{44.64} &
%   \textbf{53.48} &
%   \textbf{56.78} &
%   \textbf{59.59} &
%   \textbf{58.97} &
%   \textbf{64.93} &
%   \textbf{65.05} \\
% Llama 3 8B-Instruct &
%   25.46 &
%   4.13 &
%   2.62 &
%   3.47 &
%   4.44 &
%   15.73 &
%   51.90 &
%   58.61 \\
% Llama 3 8B-Instruct + Template &
%   54.87 &
%   16.45 &
%   27.94 &
%   31.32 &
%   30.80 &
%   34.18 &
%   44.04 &
%   50.12 \\ \midrule
% Mistral 7B &
%   \textbf{60.68} &
%   \textbf{58.67} &
%   \textbf{59.15} &
%   \textbf{58.87} &
%   \textbf{60.49} &
%   \textbf{62.02} &
%   \textbf{64.16} &
%   \textbf{65.92} \\
% Mistral 7B-Instruct &
%   47.18 &
%   48.85 &
%   52.31 &
%   54.72 &
%   55.90 &
%   56.97 &
%   59.06 &
%   60.60 \\
% Mistral 7B-Instruct + Template &
%   49.30 &
%   45.88 &
%   50.22 &
%   52.42 &
%   53.73 &
%   54.37 &
%   57.56 &
%   58.31 \\ \midrule
% Falcon 7B &
%   \textbf{41.12} &
%   \textbf{41.64} &
%   \textbf{43.11} &
%   \textbf{43.69} &
%   \textbf{44.22} &
%   \textbf{45.60} &
%   \textbf{46.35} &
%   \textbf{48.24} \\
% Falcon 7B-Instruct &
%   27.83 &
%   33.19 &
%   36.52 &
%   36.46 &
%   37.71 &
%   38.42 &
%   38.83 &
%   39.33 \\ \bottomrule
% \end{tabular}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[ht]
\centering
\caption{TriviaQA plain}
\label{tab:trivia_first}
\begin{tabular}{@{}l|rrrrrrr@{}}
\toprule
\multicolumn{1}{c|}{\textbf{TriviaQA}} & \multicolumn{7}{c}{\textbf{\# Retrieved Documents}}                                                                  \\ \midrule
\multicolumn{1}{c|}{\textbf{Model}} &
  \multicolumn{1}{c}{1} &
  \multicolumn{1}{c}{2} &
  \multicolumn{1}{c}{3} &
  \multicolumn{1}{c}{4} &
  \multicolumn{1}{c}{5} &
  \multicolumn{1}{c}{8} &
  \multicolumn{1}{c}{10} \\ \midrule
Llama 2 7B                             & \textbf{55.85} & \textbf{57.15} & \textbf{59.28} & \textbf{60.40} & \textbf{61.24} & \textbf{62.93} & \textbf{63.89} \\
Llama 2 7B-Chat                        & 32.59          & 34.63          & 41.09          & 42.95          & 46.14          & 49.19          & 48.96          \\
Llama 2 7B-Chat + Template             & 23.35          & 21.63          & 21.13          & 17.70          & 18.05          & 22.30          & 25.68          \\ \midrule
Llama 3 8B                             & \textbf{44.64} & \textbf{53.48} & \textbf{56.78} & \textbf{59.59} & \textbf{58.97} & \textbf{64.93} & \textbf{65.05} \\
Llama 3 8B-Instruct                    & 4.13           & 2.62           & 3.47           & 4.44           & 15.73          & 51.90          & 58.61          \\
Llama 3 8B-Instruct + Template         & 16.45          & 27.94          & 31.32          & 30.80          & 34.18          & 44.04          & 50.12          \\ \midrule
Mistral 7B                             & \textbf{58.67} & \textbf{59.15} & \textbf{58.87} & \textbf{60.49} & \textbf{62.02} & \textbf{64.16} & \textbf{65.92} \\
Mistral 7B-Instruct                    & 48.85          & 52.31          & 54.72          & 55.90          & 56.97          & 59.06          & 60.60          \\
Mistral 7B-Instruct + Template         & 45.88          & 50.22          & 52.42          & 53.73          & 54.37          & 57.56          & 58.31          \\ \midrule
Falcon 7B                              & \textbf{41.64} & \textbf{43.11} & \textbf{43.69} & \textbf{44.22} & \textbf{45.60} & \textbf{46.35} & \textbf{48.24} \\
Falcon 7B-Instruct                     & 33.19          & 36.52          & 36.46          & 37.71          & 38.42          & 38.83          & 39.33          \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/triviaqa_second_prompt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[ht]
\centering
\caption{TriviaQA with proof}
\label{tab:trivia_second}
\begin{tabular}{@{}l|ccccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{TriviaQA}} &
  \multicolumn{7}{c}{\textbf{\# Retrieved Documents}} \\ \midrule
\multicolumn{1}{c|}{\textbf{Model}} &
  {1} &
  {2} &
  {3} &
  {4} &
  {5} &
  {8} &
  {10} \\ \midrule
Llama 2 7B &
  {\textbf{54.94}} &
  {\textbf{56.94}} &
  {\textbf{58.88}} &
  {\textbf{60.07}} &
  {\textbf{60.87}} &
  {\textbf{62.75}} &
  {\textbf{63.73}} \\
Llama 2 7B-Chat &
  {41.86} &
  {47.18} &
  {49.53} &
  {51.19} &
  {52.59} &
  {55.73} &
  {56.00} \\
Llama 2 7B-Chat + Template &
  {4.22} &
  {6.55} &
  {8.75} &
  {10.15} &
  {14.90} &
  {20.69} &
  {27.48} \\ \midrule
Llama 3 8B &
  {\textbf{61.57}} &
  {\textbf{63.32}} &
  {\textbf{64.56}} &
  {\textbf{65.93}} &
  {\textbf{66.52}} &
  {\textbf{67.67}} &
  {\textbf{68.04}} \\
Llama 3 8B-Instruct &
  {42.67} &
  {44.44} &
  {47.11} &
  {48.10} &
  {48.71} &
  {52.59} &
  {56.48} \\
Llama 3 8B-Instruct + Template &
  {30.52} &
  {36.89} &
  {31.11} &
  {33.17} &
  {38.08} &
  {33.69} &
  {23.42} \\ \midrule
Mistral 7B &
  {\textbf{57.98}} &
  {\textbf{60.49}} &
  {\textbf{62.18}} &
  {\textbf{63.70}} &
  {\textbf{65.23}} &
  {\textbf{67.04}} &
  {\textbf{67.44}} \\
Mistral 7B-Instruct &
  {48.51} &
  {52.60} &
  {54.79} &
  {56.05} &
  {56.91} &
  {58.80} &
  {59.54} \\
Mistral 7B-Instruct + Template &
  {33.73} &
  {33.21} &
  {35.47} &
  {36.57} &
  {34.98} &
  {42.39} &
  {48.45} \\ \midrule
Falcon 7B &
  {\textbf{40.32}} &
  {\textbf{42.76}} &
  {\textbf{44.92}} &
  {\textbf{45.45}} &
  {\textbf{46.47}} &
  {\textbf{47.23}} &
  {\textbf{48.57}} \\
Falcon 7B-Instruct &
  {33.54} &
  {35.69} &
  {37.50} &
  {38.09} &
  {39.02} &
  {41.08} &
  {42.95} \\ \bottomrule
\end{tabular}
\end{table*}










% \begin{table*}[ht]
% \centering
% \small
% \caption{TriviaQA with proof}
% \begin{tabular}{@{}l|lllllll@{}}
% \toprule
% \textbf{TriviaQA} & \multicolumn{7}{c}{\textbf{\# Retrieved Documents}} \\ \midrule
% \textbf{Model} & 1 & 2 & 3 & 4 & 5 & 8 & 10 \\ \midrule
% Llama 2 7B &
%   \textbf{54.94}$_{37.22\%}$ &
%   \textbf{56.94}$_{44.27\%}$ &
%   \textbf{58.88}$_{44.68\%}$ &
%   \textbf{60.07}$_{47.19\%}$ &
%   \textbf{60.87}$_{48\%}$ &
%   \textbf{62.75}$_{50.35\%}$ &
%   \textbf{63.73}$_{47.14\%}$ \\
% Llama 2 7B-Chat &
%   41.86$_{43.15\%}$ &
%   47.18$_{49.61\%}$ &
%   49.53$_{53.09\%}$ &
%   51.19$_{53.46\%}$ &
%   52.59$_{48.92\%}$ &
%   55.73$_{40.14\%}$ &
%   56.00$_{28.93\%}$ \\
% Llama 2 7B-Chat + Template &
%   4.22$_{0.05\%}$ &
%   6.55$_{0.46\%}$ &
%   8.75$_{0.75\%}$ &
%   10.15$_{0.11\%}$ &
%   14.90$_{0.04\%}$ &
%   20.69$_{0\%}$ &
%   27.48$_{0\%}$ \\ \midrule
% Llama 3 8B &
%   \textbf{61.57}$_{51.66\%}$ &
%   \textbf{63.32}$_{57.44\%}$ &
%   \textbf{64.56}$_{59.46\%}$ &
%   \textbf{65.93}$_{61.30\%}$ &
%   \textbf{66.52}$_{62.02\%}$ &
%   \textbf{67.67}$_{64.12\%}$ &
%   \textbf{68.04}$_{63.58\%}$ \\
% Llama 3 8B-I &
%   42.67$_{35.45\%}$ &
%   44.44$_{50.55\%}$ &
%   47.11$_{50.89\%}$ &
%   48.10$_{48.91\%}$ &
%   48.71$_{55.02\%}$ &
%   52.59$_{55.28\%}$ &
%   56.48$_{56.78\%}$ \\
% Llama 3 8B-I + Template &
%   30.52$_{1.10\%}$ &
%   36.89$_{0.13\%}$ &
%   31.11$_{0.12\%}$ &
%   33.17$_{0.49\%}$ &
%   38.08$_{1.59\%}$ &
%   33.69$_{1.42\%}$ &
%   23.42$_{0.5\%}$ \\ \midrule
% Mistral 7B &
%   \textbf{57.98}$_{43.23\%}$ &
%   \textbf{60.49}$_{52.16\%}$ &
%   \textbf{62.18}$_{56.07\%}$ &
%   \textbf{63.70}$_{58.48\%}$ &
%   \textbf{65.23}$_{60.82\%}$ &
%   \textbf{67.04}$_{66.66\%}$ &
%   \textbf{67.44}$_{68.04\%}$ \\
% Mistral 7B-I &
%   48.51$_{51.08\%}$ &
%   52.60$_{53.52\%}$ &
%   54.79$_{55.43\%}$ &
%   56.05$_{57.53\%}$ &
%   56.91$_{58.55\%}$ &
%   58.80$_{59.68\%}$ &
%   59.54$_{58.58\%}$ \\
% Mistral 7B-I + Template &
%   33.73$_{16.82\%}$ &
%   33.21$_{14.87\%}$ &
%   35.47$_{11.42\%}$ &
%   36.57$_{7.90\%}$ &
%   34.98$_{5.70\%}$ &
%   42.39$_{2.45\%}$ &
%   48.45$_{2.16\%}$ \\ \midrule
% Falcon 7B &
%   \textbf{40.32}$_{3.02\%}$ &
%   \textbf{42.76}$_{3.70\%}$ &
%   \textbf{44.92}$_{3.47\%}$ &
%   \textbf{45.45}$_{4.52\%}$ &
%   \textbf{46.47}$_{4.86\%}$ &
%   \textbf{47.23}$_{3.17\%}$ &
%   \textbf{48.57}$_{1.61\%}$ \\
% Falcon 7B-I &
%   33.54$_{4.45\%}$ &
%   35.69$_{5.94\%}$ &
%   37.50$_{6.53\%}$ &
%   38.09$_{6.08\%}$ &
%   39.02$_{6.28\%}$ &
%   41.08$_{3.34\%}$ &
%   42.95$_{1.67\%}$ \\
% \bottomrule
% \end{tabular}
% \end{table*}




==> tables/triviaqa_second_prompt_coherence.tex <==

\begin{table*}[ht]
\centering
\label{tab:trivia_second_coherence}
\caption{Trivia QA coherence percentage with proof}
\begin{tabular}{@{}l|lllllll@{}}
\toprule
\multicolumn{1}{c|}{\textbf{TriviaQA}} & \multicolumn{7}{c}{\textbf{\# Retrieved Documents}}                                                                  \\ \midrule
\multicolumn{1}{c|}{\textbf{Model}} &
  \multicolumn{1}{c}{1} &
  \multicolumn{1}{c}{2} &
  \multicolumn{1}{c}{3} &
  \multicolumn{1}{c}{4} &
  \multicolumn{1}{c}{5} &
  \multicolumn{1}{c}{8} &
  \multicolumn{1}{c}{10} \\ \midrule
Llama 2 7B                             & 37.22          & 44.27          & 44.68          & 47.19          & 48.00          & \textbf{50.35} & \textbf{47.14} \\
Llama 2 7B-Chat                        & \textbf{43.15} & \textbf{49.61} & \textbf{53.09} & \textbf{53.46} & \textbf{48.92} & 40.14          & 28.93          \\
Llama 2 7B-Chat + Template             & 0.05           & 0.46           & 0.75           & 0.11           & 0.04           & 0              & 0              \\ \midrule
Llama 3 8B                             & \textbf{51.66} & \textbf{57.44} & \textbf{59.46} & \textbf{61.30} & \textbf{62.02} & \textbf{64.12} & \textbf{63.58} \\
Llama 3 8B-Instruct                    & 35.45          & 50.55          & 50.89          & 48.91          & 55.02          & 55.28          & 56.78          \\
Llama 3 8B-Instruct + Template         & 1.10           & 0.13           & 0.12           & 0.49           & 1.59           & 1.42           & 0.5            \\ \midrule
Mistral 7B                             & 43.23          & 52.16          & \textbf{56.07} & \textbf{58.48} & \textbf{60.82} & \textbf{66.66} & \textbf{68.04} \\
Mistral 7B-Instruct                    & \textbf{51.08} & \textbf{53.52} & 55.43          & 57.53          & 58.55          & 59.68          & 58.58          \\
Mistral 7B-Instruct + Template         & 16.82          & 14.87          & 11.42          & 7.90           & 5.70           & 2.45           & 2.16           \\ \midrule
Falcon 7B                              & 3.02           & 3.70           & 3.47           & 4.52           & 4.86           & 3.17           & 1.61           \\
Falcon 7B-Instruct                     & \textbf{4.45}  & \textbf{5.94}  & \textbf{6.53}  & \textbf{6.08}  & \textbf{6.28}  & \textbf{3.34}  & \textbf{1.67}  \\ \bottomrule
\end{tabular}
\end{table*}
